Reflow: Automatically Improving Touch Interactions in Mobile Applications through Pixel-based Refinements

Touch is the primary way that users interact with smartphones. However, building mobile user interfaces where touch interactions work well for all users is a difficult problem, because users have different abilities and preferences. We propose a system, Reflow, which automatically applies small, personalized UI adaptations, called refinements -- to mobile app screens to improve touch efficiency. Reflow uses a pixel-based strategy to work with existing applications, and improves touch efficiency while minimally disrupting the design intent of the original application. Our system optimizes a UI by (i) extracting its layout from its screenshot, (ii) refining its layout, and (iii) re-rendering the UI to reflect these modifications. We conducted a user study with 10 participants and a heuristic evaluation with 6 experts and found that applications optimized by Reflow led to, on average, 9% faster selection time with minimal layout disruption. The results demonstrate that Reflow's refinements useful UI adaptations to improve touch interactions.

==> Reflow EICS 2022_arXiv_arXiv/table_heuristic.tex <==
\newcommand{\heplusone}{\cellcolor{blue!10}$+1$}
\newcommand{\heplustwo}{\cellcolor{blue!20}$+2$}
\newcommand{\heplusthree}{\cellcolor{blue!30}$+3$}
\newcommand{\heplusfour}{\cellcolor{blue!40}$+4$}

\newcommand{\hezero}{\cellcolor{gray!5}}
\newcommand{\heblank}{\cellcolor{white}$\cdot$}

\newcommand{\heminusone}{\cellcolor{orange!10}$-1$}
\newcommand{\heminustwo}{\cellcolor{orange!20}$-2$}
\newcommand{\heminusthree}{\cellcolor{orange!30}$-3$}
\newcommand{\heminusfour}{\cellcolor{orange!40}$-4$}

\begin{table}[t]
\centering
\begin{threeparttable}
\caption{Relative Likert Scores for Heuristic Evaluation}
\begin{tabulary}{\linewidth}{Lcccccc}
\toprule
& \multicolumn{3}{c}{AX} & \multicolumn{3}{c}{DS} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
Heuristic & E1 & E2 & E3 & E4 & E5 & E6\\
\midrule
\textsc{Alignment} & 
  \heminusone & 
  \hezero & 
  \heminusone & 
  \heminusone & %
  \heplusone & 
  \heminusone
\\
\textsc{Selection Time} &
  \heplusone &
  \heplusone &
  \heplusone &
  \hezero &
  \heplusone &
  \heplusone
\\
\textsc{Clutter} &
  \hezero &
  \heminusone & 
  \heminustwo &
  \heminusone & 
  \heplustwo &
  \heminusone 
\\
\textsc{Saliency} &
  \heminusone &
  \heplusone & 
  \hezero &
  \heminusone & 
  \heplusone &
  \heminusone 
\\
\textsc{Grouping} &
  \heminusone &
  \hezero & 
  \heminusone &
  \hezero & 
  \heplusone &
  \hezero
\\

\bottomrule
\end{tabulary}
\label{tab:heuristic_eval}
\begin{tablenotes}
\item Expert evaluations from heuristic evaluation. Ratings are normalized to show deviation from the neutral option (``About the same (3)"). Positive scores indicate better change and negative scores indicate worse change. AX denotes accessibility expert while DS denotes design expert.
\end{tablenotes}
\end{threeparttable}
\end{table}

